Regional Modelling of the Southern African Geomagnetic Field using Harmonic Splines

Over the southern African region the geomagnetic field is weak and changes rapidly. For this area series of geomagnetic field measurements exist since the 1950s. We take advantage of the existing repeat station surveys and observatory annual means, and clean these data sets by eliminating jumps and minimising external field contributions in the original time series. This unique data set allows us to obtain a detailed view of the geomagnetic field behaviour in space and time by computing a regional model. For this, we use a system of representation similar to harmonic splines. Initially, the technique is systematically tested on synthetic data. After systematically testing the method on synthetic data, we derive a model for 1961 to 2001 that gives a detailed view of the fast changes of the geomagnetic field in this region.

==> journal_abbrev.tex <==
%--- definition of iso abbreviations ---%

% to include the file in your LaTeX document use \input{journal_abbrev_L}

%--- last changes ---%
% 2008/11/15, Daniel Heisselmann: Initial document

%\newcommand{\}{}
\newcommand{\actaa}{Acta Astronomica}
\newcommand{\ao}{Applied Optics}
\newcommand{\aap}{Astronomy and Astrophysics}
\newcommand{\aapr}{Astronomy and Astrophysics Reviews}
\newcommand{\aj}{The Astronomical Journal}
\newcommand{\apj}{The Astrophysical Journal}
\newcommand{\apjl}{The Astrophysical Journal, Letters to the Editor}
\newcommand{\apjs}{The Astrophysical Journal, Supplement Series}
\newcommand{\aplett}{Astrophysics Letters and Communications}
\newcommand{\apspr}{Astrophysics Space Physics Research}
\newcommand{\apss}{Astrophysics and Space Science}
\newcommand{\aaps}{Astrophysics and Space Science, Supplement Series}
\newcommand{\araa}{Annual Review of Astronomy and Astrophysics}
\newcommand{\gca}{Geochimica Cosmochimica Acta}
\newcommand{\grl}{Geophysical Research Letters}
\newcommand{\icarus}{Icarus}
\newcommand{\mnras}{The Monthly Notices of the Royal Astronomical Society}
\newcommand{\jcp}{Journal of Chemical Physics}
\newcommand{\jcis}{Journal of Colloid and Interface Science}
\newcommand{\jfm}{Journal of Fluid Mechanics}
\newcommand{\jgr}{Journal of Geophysical Research}
\newcommand{\planss}{Planetary and Space Science}
\newcommand{\nat}{Nature}
\newcommand{\prl}{Physical Review Letters}
\newcommand{\pra}{Physical Review A}
\newcommand{\prb}{Physical Review B}
\newcommand{\prc}{Physical Review C}
\newcommand{\prd}{Physical Review D}
\newcommand{\pre}{Physical Review E}
\newcommand{\rsi}{Review of Scientific Instruments}
\newcommand{\solphys}{Solar Physics}
\newcommand{\ssr}{Space Science Reviews}
\newcommand{\zap}{Zeitschrift f{\"u}r Astronomie} 
